Following High-level Navigation Instructions on a Simulated Quadcopter with Imitation Learning

We introduce a method for following high-level navigation instructions by mapping directly from images, instructions and pose estimates to continuous low-level velocity commands for real-time control. The Grounded Semantic Mapping Network (GSMN) is a fully-differentiable neural network architecture that builds an explicit semantic map in the world reference frame by incorporating a pinhole camera projection model within the network. The information stored in the map is learned from experience, while the local-to-world transformation is computed explicitly. We train the model using DAggerFM, a modified variant of DAgger that trades tabular convergence guarantees for improved training speed and memory use. We test GSMN in virtual environments on a realistic quadcopter simulator and show that incorporating an explicit mapping and grounding modules allows GSMN to outperform strong neural baselines and almost reach an expert policy performance. Finally, we analyze the learned map representations and show that using an explicit map leads to an interpretable instruction-following model.

==> future.tex <==
\section{Future Work}
\label{sec:future}

\ya{This section is candidate for removal -- often easy to fold into conclusion, especially for submission}

==> task.tex <==
\section{Task}
\label{sec:task}

We model visual navigation for instruction following as a sequential decision-making process \cite{duvallet2013imitation}. Initially at timestep $t=0$ the agent controlled by a policy $\pi$ receives an utterance $u$ describing the navigation objective. Thereafter, at each timestep $t \geq 0$ the policy visits a state $s_t \in \mathcal{S}$, observes an observation $o_t = \mathcal{O}(s_t)$ and executes an action $a_t \in \mathcal{A}$:

$$a_t \sim \pi(o_t, u)$$

The environment then transitions to state $s_{t+1} \sim \mathcal{T}(s_t, a_t)$ and produces a new observation $o_{t+1} = \mathcal{O}(s_{t+1})$.

In our quadcopter visual navigation task, the action $a = (v^x, v^\omega, p^{stop})$ is a tuple containing the target forward and yaw velocity targets as well as stopping probability $\stopprob$. The observation $o_t = [I_t, x_t, q_t]$ consists of the first-person camera image $I_t$ and the quadcopter's position and orientation estimates $x_t$ and $q_t$. \rk{It's unintuitive that $v^x$ and $x_t$ are parallel but $v^\omega$ and $q_t$ are not.  Usually $q$ is configuration.  Could this be $\theta$?}
The environment $\mathcal{T}$ is defined by the Microsoft AirSim simulator \cite{airsim2017fsr}. 
The full environment state $s_t = [x^*_t, q^*_t, \{O_j\}, G, s_{s}, \gamma_u]$ includes the quadcopter's true location, the set of all present object locations $\{O_j\}$, the goal location $G$ and the simulator's internal state $s_s$ which is inaccessible. 
The observation $o_t$ is rendered using the Unreal Engine's renderer $\mathcal{O} : \mathcal{S} \rightarrow \mathcal{O}$.\\

The task of the policy $\pi$ is to produce a sequence of actions $a_t$, such that the resulting position-action trajectory $\Xi_\pi = (x_0, a_0, x_1, a_1, ... , x_T, a_T)$ terminates with a stop action in a location $x_T$ close to the ground-truth goal location $G$.

\[\texttt{success}(\Xi_\pi) := 
\begin{cases}
true,& \|x^*_T - G \|_2 < D_T \wedge p^{stop}_T > 0.5\\
false,& \text{otherwise}
\end{cases}
\
\]

We assume availability of an expert policy $\pi^*$ at training time only. The expert has access to the ground-truth trajectory $\Xi_u$, which represents the meaning of the instruction $u$. This assumption is commonly satisfiable in natural-language instruction following tasks \textbf{(cite a few)}. At every timestep, the expert policy produces a ground-truth action label using a simple path-following carrot planner tuned to the robot dynamics:

$$a^*_t = \pi^*(o_t, \Xi_u)$$

We train the policy $\pi$ to mimic the expert $\pi^*$ using Imitation Learning. We perform Nonlinear Logistic Regression with respect to the stopping probability $p^{stop}$ and Least-Squares regression with respect to the velocities $v^x$ and $v^\omega$. Formally, we minimize the expected distance between the expert action $a^*$ and the policy action on the state distribution $d_\pi$ induced by the learned policy $\pi$:

\begin{equation}
J_{action}(\pi)_{s_t \sim d_\pi} =  \mathbb{E}[D_a(\pi(o_t, u), \pi^*(o_t, \Xi_u))]
\label{eq:main_objective}
\end{equation}

Where the distance metric between actions is defined as:

\begin{equation}
\begin{split}
D_a(a, a^*) = \lambda_x \|v^x - v^{*x}\|^2_2 + \lambda_\omega \|v^\omega - v^{*\omega}\|^2_2 + \\
 \lambda_{stop} [p^{*stop}log(p^{stop}) + (1 - p^{*stop})log(1 - p^{stop})]
\end{split}
\end{equation}

The hyperparameters $\lambda_x$, $\lambda_\omega$, $\lambda_{stop}$ are useful to place more emphasis on turning and stopping, which are essential for navigation success, while placing less importance on predicting the correct velocity. We've chosen $\lambda_x$ = 0.2, $\lambda_\omega$ = 0.4, $\lambda_{stop}$ = 0.4, but we found that the task performance is not highly sensitive to this choice and one could just set $\lambda_x = \lambda_\omega = \lambda_{stop} = 1$.

